CoLT5: Faster Long-Range Transformers with Conditional Computation

Many natural language processing tasks benefit from long inputs, but processing long documents with Transformers is expensive -- not only due to quadratic attention complexity but also from applying feedforward and projection layers to every token. However, not all tokens are equally important, especially for longer documents. We propose CoLT5, a long-input Transformer model that builds on this intuition by employing conditional computation, devoting more resources to important tokens in both feedforward and attention layers. We show that CoLT5 achieves stronger performance than LongT5 with much faster training and inference, achieving SOTA on the long-input SCROLLS benchmark. Moreover, CoLT5 can effectively and tractably make use of extremely long inputs, showing strong gains up to 64k input length.

==> figures/conbo.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.99\textwidth]{images/conbo}
    \caption{An overview of a \slic Transformer layer with conditional computation.}
    \label{fig:conbo}
\end{figure*}

==> figures/few_shot.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \begin{tikzpicture}[scale=1.0]
            \begin{axis}[
            scale only axis,
            width=0.8\textwidth,
            height=0.5\textwidth,
            ylabel={Exact Match},
            % ylabel shift=-3pt,            
            xlabel={Number of shots},
            mark=x,
            xmode=log,
            % log ticks with fixed point,
            x tick label style={log ticks with fixed point},
            ymajorgrids=true,
            xmajorgrids=true,
            xminorticks=true,
            grid style=dashed,
            % ymin=30,
            % ymax=44,        
            % ticklabel style = {font=\small}
            legend pos={north west},
            ylabel style={align=left, text height=0.2cm},
            % legend style={font=\large},
            ]
            \addlegendimage{empty legend}\addlegendentry{TriviaQA}
            \addplot[color=longtcolor,mark=\longtmark,mark size=2pt, line width=2] table {
                % base
                34.60595312 60.55
            };
            \addplot[color=sliccolor,mark=\modelmark,mark size=3pt, line width=2] table {
                % base
                6.00157812  61.40
            };
            \end{axis}
        \end{tikzpicture}  
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \begin{tikzpicture}[scale=1.0]
            \begin{axis}[
            scale only axis,
            width=0.8\textwidth,
            height=0.5\textwidth,
            % ylabel={Exact Match},
            % ylabel shift=-3pt,            
            xlabel={Number of shots},
            mark=x,
            xmode=log,
            % log ticks with fixed point,
            x tick label style={log ticks with fixed point},
            ymajorgrids=true,
            xmajorgrids=true,
            xminorticks=true,
            grid style=dashed,
            % ymin=30,
            % ymax=44,        
            % ticklabel style = {font=\small}
            legend pos={north west},
            ylabel style={align=left, text height=0.2cm},
            % legend style={font=\large},
            ]
            \addlegendimage{empty legend}\addlegendentry{Placeholder}
            \addplot[color=longtcolor,mark=\longtmark,mark size=2pt, line width=2] table {
                % base
                34.60595312 60.55
            };
            \addplot[color=sliccolor,mark=\modelmark,mark size=3pt, line width=2] table {
                % base
                6.00157812  61.40
            };
            \end{axis}
        \end{tikzpicture}  
     \end{subfigure}
     \hfill
     \begin{tikzpicture}
        \begin{customlegend}[
            legend columns=2,
            legend style={
                align=center,
                column sep=4ex,
                font=\large,
            },
            legend entries={\longt, \slic}
        ]
        \addlegendimage{mark=\longtmark,mark size=3pt,solid,color=longtcolor}          
        \addlegendimage{mark=\modelmark,solid,color=sliccolor}
     
        \end{customlegend}
    \end{tikzpicture}            
    \caption{K-shot performance on TriviaQA and PLACEHOLDER as a function of number of shots for \slic and \longt XL models.}
    \label{fig:few_shot}
\end{figure*}
